Rational Economic Behaviours in the Bitcoin Lightning Network

The Bitcoin Lightning Network (LN) is designed to improve the scalability of blockchain systems by using off-chain payment paths to settle transactions in a faster, cheaper, and more private manner. This work aims to empirically study LN's fee revenue for network participants. Under realistic assumptions on payment amounts, routing algorithms and traffic distribution, we analyze the economic returns of the network's largest routing nodes which currently hold the network together, and assess whether the centralizing tendency is incentive-compatible from an economic viewpoint. Moreover, since recent literature has proved that participation is economically irrational for the majority of large nodes, we evaluate the long-term impact on the network topology when participants start behaving rationally.

==> extra.tex <==
\section{Empirical analysis: Short term impact of random strategy}
The final result we want to highlight is network equilibrium. As we can see from [table ...], even imposing random new fees, or with random channel selection nodes could increase their fee revenue. Of course, there is the important aspect of keeping channels balanced that cannot be overlooked, but from the previous analysis, nodes seem to have not yet policies that allow them to maximize their profits.

\subsection{Methodology}
To better illustrate our findings we highlight now that even the random strategy allows nodes to earn more. 
We randomly picked 100 nodes out of 1,000 and we randomly changed first their fee in the first result, and then their neighbors but keeping the same capacity in the second one. The results show that even by randomly changing their configuration, they can increase their ratio by many orders of magnitude. This leads us to think that nodes' fees are not yet optimal for revenue and more research is required into channel selection strategies. 
The framework to get the result is the following:
\begin{enumerate}
    \item Simulate payments in the network
    \item Pick a node \(u \in U\) uniformly at random.
    \item Change node \(u\) \(fee_e\) for each of its channels \(e_{uw}\) where \(w \in N(u)\)
    \item Run a new simulation to compare the results
\end{enumerate}


\subsection{Random Channel - dual funded}
In this second type of experiment, we proceeded as follows. We randomly picked a set of nodes to which we changed the channels but maintaining the same fee. All the previous channels of the nodes were closed. And the same number of channels were reopened with different nodes. The capacity of the closed channels is the same as the capacity of the newly created channels. For node $u$ to open a channel with node $w$, after closing a channel with node $v$, node $w$ needs to satisfy the following condition:
\[
\frac{c_{uv}}{2 \cdot \deg^+(u)} < \min(c_{wz_1}, c_{wz_2}, \ldots, c_{wz_n})
\]
where $n$ is the number of neighbor of $w$ and $z$ is a neighbor of $w$. This way node $w$ can commit part of the liquidity in its channels to open the new channel with $u$. At the same time, when closing a channel half of the capacity of the closing channel is uniformly distributed to the other channels of node $v$.
